The IRX-Beta Relation in kpc-sized Star Forming Regions in Nearby Galaxies

The effect of dust attenuation on a galaxy's light depends on a number of physical properties, such as geometry and dust composition, both of which can vary across the faces of galaxies. To investigate this variation, we continue analysis on star-forming regions in 29 galaxies studied previously. We analyse these regions using Swift/UVOT and WISE images, as well as SDSS/MaNGA emission line maps to constrain the relationship between the infrared excess (IRX) and the UV spectral index (beta) for each star forming region. This relationship can be used to constrain which dust attenuation law is appropriate for the region. We find that the value of Dn(4000) for a region is correlated with both IRX and beta, and that the gas-phase metallicity is strongly correlated with the IRX. This correlation between metallicity and IRX suggests that regardless of aperture, metal rich regions have steeper attenuation curves. We also find that integrated galactic light follows nearly the same IRX-beta relationship as that found for kiloparsec-sized star forming regions. This similarity may suggest that the attenuation law followed by the galaxy is essentially the same as that followed by the regions, although the relatively large size of our star forming regions complicates this interpretation because optical opacity and attenuation curves have been observed to vary within individual galaxies.

==> Tables/region_comparison.tex <==
\begin{table*}
%\centering
\caption{Molina+20 versus Duffy+23 regions.}\label{table:region_comp}
\setlength{\tabcolsep}{17 pt}
\begin{tabular}{cc}
\hline\hline
Molina+20 & Duffy+23\\
Region & Region\\
I.D. & I.D.\\
(1) & (2) \\
\hline
1.1 & Included in 1.1 \\
1.2 & Included in 1.1 \\
1.3 & Included in 1.1 \\
2.1 & Matches 2.1 \\
3.1 & Matches 3.1 \\
4.1 & Matches 4.1 \\
5.1 & Matches 5.1 \\
6.1 & Matches 6.1 \\
7.1 & Included in 7.1 \\
7.2 & Included in 7.1 \\
7.3 & Included in 7.1 \\
8.1 & Matches 8.1 \\
9.1 & Included in 9.1 \\
9.2 & Included in 9.1 \\
9.3 & Included in 9.1 \\
10.1 & Included in 10.1 \\
10.2 & Included in 10.1 \\
11.1 & Included in 11.1 \\
12.1 & Included in 12.1 \\
12.2 & Included in 12.1 \\
12.3 & Included in 12.1\\
13.1 & Matches 13.1 \\
13.2 & Not resolved \\
13.3 & Matches 13.2\\
14.1 & Matches 14.1 \\
15.1 & Included in 15.1 \\
16.1 & Included in 16.1 \\
16.2 & Included in 16.1 \\
17.1 & Matches 17.1 \\
18.1 & Matches 18.1 \\
19.1 & Included in 19.1 \\
20.1 & Matches 20.2 \\
20.2 & Not resolved \\
20.3 & Matches 20.1\\
21.1 & Matches 21.1 \\
22.1 & Matches 22.1 \\
23.1 & Included in 23.2\\
23.2 & Included in 23.2 \\
23.3 & Not resolved \\
23.4 & Matches 23.1\\
24.1 & Included in 24.1 \\
24.2 & Included in 24.1 \\
25.1 & \\
25.2 & \\
25.3 & \\
25.4 & \\
25.5 & \\
25.6 & \\
26.1 & 154.7685 & 46.4544 & 6.0 & 1.0 & \dots \\
26.2 & 154.7715 & 46.4515 & 10.0 & 0.4 & 90 \\
26.3\\
26.4\\
26.5\\
27.1 & 176.1242 & 55.5785 & 8.0 & 0.5 & 0 \\
28.1 & 113.4005 & 45.9434 & 6.0 & 1.0 & \dots \\
29.1 & 46.7171 & $-0.8966$ & 6.0 & 1.0 & \dots \\
\hline
\end{tabular}
\\ Column 1: Region I.D. from \cite{2020MNRAS.494.4751M}. Column 2: Where the region falls within the newly identified regions in this work. Included in means that some or all of the \cite{2020MNRAS.494.4751M} region is included in the newly identified region, matches means that the region is either exactly matched to the new region, or that the new region is located at nearly the same place and only includes that region, and not resolved means we do not recover the region at the lower resolution.
\end{table*}
